Learning an Unknown Network State in Routing Games

We study learning dynamics induced by myopic travelers who repeatedly play a routing game on a transportation network with an unknown state. The state impacts cost functions of one or more edges of the network. In each stage, travelers choose their routes according to Wardrop equilibrium based on public belief of the state. This belief is broadcast by an information system that observes the edge loads and realized costs on the used edges, and performs a Bayesian update to the prior stage's belief. We show that the sequence of public beliefs and edge load vectors generated by the repeated play converge almost surely. In any rest point, travelers have no incentive to deviate from the chosen routes and accurately learn the true costs on the used edges. However, the costs on edges that are not used may not be accurately learned. Thus, learning can be incomplete in that the edge load vectors at rest point and complete information equilibrium can be different. We present some conditions for complete learning and illustrate situations when such an outcome is not guaranteed.

==> self_confirm.tex <==
%!TEX root = ifacconf.tex% of learning dynamics that converge to self-confirming equilibrium and Nash equilibrium. %We first present examples where learning leads to a Nash equilibrium, and discuss how the number of states, network topology and the randomness of the realized travel time effect the learning speed. We then show an example where learning leads to a self-confirming equilibrium with one initial belief, but leads to a Nash equilibrium given another initial belief. 


%In this example, Assumptions \ref{continuity} - \ref{bound_alpha} are all satisfied. 
%
%In the following example, we show that the learning speed is faster if the number of possible states decreases. 
%\begin{example}\label{example_three}
%We consider the same game in Example \ref{benchmark}, except that the state set is $\{e_1, e_3, \emptyset\}$, and the initial belief changes to the follows: 
%\[\ps(e_1)=1/6, \quad \ps(e_3)=1/3, \quad \ps(\emptyset)=1/2.\]
%Fig. \ref{three_1}-\ref{three_4} show how the belief of each state changes as $\t$ grows from 0 to 1000. 
%\begin{figure}[H]
%    \begin{subfigure}[b]{0.31 \textwidth}
%        \includegraphics[width=\textwidth]{state_1_three.eps}
%        \caption{$\sran=e_1$.}
%        \label{three_1}
%    \end{subfigure}
%~
%\centering
%	\begin{subfigure}[b]{0.31\textwidth}
%        \includegraphics[width=\textwidth]{state_3_three.eps}
%        \caption{$\sran=e_3$.}
%        \label{three_2}
%    \end{subfigure}
%    ~
%   \begin{subfigure}[b]{0.31\textwidth}
%        \includegraphics[width=\textwidth]{state_4_three.eps}
%        \caption{$\sran=\emptyset$.}
%        \label{three_4}
%    \end{subfigure}
%    \caption{Rational learning converges to Nash equilibrium, $\S=\{e_1, e_3, \emptyset\}$}
%\label{fig:correct_prior_converge}
%\end{figure}
%\end{example}
%
%Additionally, we show that if the realized travel time becomes more noisy, then the learning speed becomes slower. 
%\begin{example}\label{example_noisy}
%We consider the same game in Example \ref{benchmark}, except that $\epe \sim U[-5, 5]$ for all $\e \in \E$. Fig. \ref{theta_1_noisy}-\ref{theta_4_noisy} show how the belief of each state changes as $\t$ grows from 0 to 3000. 
%\begin{figure}[H]
%    \begin{subfigure}[b]{0.40 \textwidth}
%        \includegraphics[width=\textwidth]{theta_1_noisy.eps}
%        \caption{$\sran=e_1$.}
%        \label{theta_1_noisy}
%    \end{subfigure}
%~
%\centering
%	\begin{subfigure}[b]{0.40\textwidth}
%        \includegraphics[width=\textwidth]{theta_2_noisy.eps}
%        \caption{$\sran=e_2$.}
%        \label{theta_2_noisy}
%    \end{subfigure}\\
%   \begin{subfigure}[b]{0.40\textwidth}
%        \includegraphics[width=\textwidth]{theta_3_noisy.eps}
%        \caption{$\sran=e_3$.}
%        \label{theta_3_noisy}
%    \end{subfigure}
%~
%\centering
%	\begin{subfigure}[b]{0.40\textwidth}
%        \includegraphics[width=\textwidth]{theta_4_noisy.eps}
%        \caption{$\sran=\emptyset$.}
%        \label{theta_4_noisy}
%    \end{subfigure}
%    \caption{Rational learning converges to Nash equilibrium, $\epe \sim U[-5, 5]$.}
%\label{fig:correct_prior_converge}
%\end{figure}
%\end{example}
%
%We summarize our observations from Examples \ref{benchmark}-\ref{example_noisy} as follows: 
%\begin{enumerate}
%\item The convergence rate of $\thetat$ is exponential in all four states. 
%\item When the state is $\s=e_1$, the learning converges with the fastest speed. This is because the information of $s=e_1$ is included in the realized cost of both routes. 
%\item The learning speed is faster if the size of $\S$ is smaller.
%\item The convergence rate is much slower when the variance of travel cost increases. 
%\end{enumerate}
%
%
%Finally, we present an example where the learning dynamics converges to a Nash equilibrium given an initial belief, but converges to a self-confirming equilibrium given another initial belief. 
%
%
%Additionally, we consider the learning dynamics with the initial belief as follows: 
%\[\ps(e_1)=1/12, \quad \ps(e_2)=1/120, \quad \ps(e_3)=1/3, \quad \ps(\emptyset)=69/120.\]
%\begin{figure}[H]
%    \begin{subfigure}[b]{0.40 \textwidth}
%        \includegraphics[width=\textwidth]{q_self_confirm_avoid.eps}
%        \caption{Markov-perfect equilibrium.}
%        \label{q_self_confirm}
%    \end{subfigure}
%~
%\centering
%	\begin{subfigure}[b]{0.40\textwidth}
%        \includegraphics[width=\textwidth]{theta_self_confirm_avoid.eps}
%        \caption{Public belief.}
%        \label{theta_self_confirm_avoid}
%    \end{subfigure}
%    \caption{Rational learning converges to Nash equilibrium.}
%\label{fig:avoid}
%\end{figure}
%\end{example}
%
%
%On the other hand, if in the initial belief, $\thetazero(e_2)$ is sufficiently small, then travelers still use both routes, and thus can get information of edge $e_2$. We can see from Fig. \ref{fig:avoid} that in such case, learning leads to a Nash equilibrium.  





